Interpretable Anomaly Detection with DIFFI: Depth-based Isolation Forest Feature Importance

Anomaly Detection is an unsupervised learning task aimed at detecting anomalous behaviours with respect to historical data. In particular, multivariate Anomaly Detection has an important role in many applications thanks to the capability of summarizing the status of a complex system or observed phenomenon with a single indicator (typically called `Anomaly Score') and thanks to the unsupervised nature of the task that does not require human tagging. The Isolation Forest is one of the most commonly adopted algorithms in the field of Anomaly Detection, due to its proven effectiveness and low computational complexity. A major problem affecting Isolation Forest is represented by the lack of interpretability, an effect of the inherent randomness governing the splits performed by the Isolation Trees, the building blocks of the Isolation Forest. In this paper we propose effective, yet computationally inexpensive, methods to define feature importance scores at both global and local level for the Isolation Forest. Moreover, we define a procedure to perform unsupervised feature selection for Anomaly Detection problems based on our interpretability method; such procedure also serves the purpose of tackling the challenging task of feature importance evaluation in unsupervised anomaly detection. We assess the performance on several synthetic and real-world datasets, including comparisons against state-of-the-art interpretability techniques, and make the code publicly available to enhance reproducibility and foster research in the field.

==> literature.tex <==
\label{sec:literature}

\subsection*{Interpretable Machine Learning}

Interpretable Machine Learning, or XAI, is a research field that is attracting great interest in the past recent years, as evidenced by a growing body of research in the field and as a consequence of the widespread interests and diffusion of Machine Learning-based applications in countless application scenarios and industries \cite{jordan2015machine}. The general goal of XAI is to shed light on the inner workings of Machine Learning (ML) and Deep Learning (DL) models, especially in the context of regression and classification problems. A major focus is put on Deep Neural Networks (DNNs) \cite{che2016interpretable} and ensemble methods \cite{tolomei2017interpretable}, two emblematic examples of algorithms classes that provide models that are highly accurate, but really hard to be understood by humans.

Given the fact that DNNs achieve state-of-the-art performance on several complex tasks such as image classification, text classification and time series forecasting, just to name a few, it comes as no surprise that a considerable volume of research in the XAI field focused on the problem of DNNs interpretability. The latter can be tackled with the purpose of either providing explanations about the predictions (i.e. the outputs) produced by the model \cite{zeiler2014visualizing, simonyan2013deep, murdoch2018beyond}, or interpreting the internal representations of the processed data \cite{sharif2014cnn, bau2017network}. It is worth highlighting a third promising line of research aimed at designing inherently interpretable DNNs \cite{melis2018towards, li2018deep, oreshkin2019n}. Since a complete dissertation on DNNs interpretability is out of the scope of this work, we refer the curious reader to \cite{gilpin2018explaining, zhang2018visual}.

As regards ensemble methods, we here mainly focus on Random Forests (RFs) \cite{breiman2001random}, but several works on the interpretation of other ensembles (such as Gradient Boosting Decision Trees) can be found in literature \cite{valdes2016mediboost, wang2018tem}. RFs are ensembles of classification or regression trees leveraging \textit{bagging} to reduce the variance of predictions. To further improve the variance decrease, RFs typically implement \textit{feature bagging}, which consists in reducing the correlation between base estimators by considering a random subset of the original feature set to grow each tree. With respect to single Decision Trees, RFs significantly improve performance in terms of accuracy, at the price of reduced interpretability. In this context, many works address the problem of improving standard feature importance score methods. Relevant examples are \cite{strobl2008conditional}, which proposes an improvement of the permutation importance measured based on a conditional permutation scheme, and \cite{li2019debiased}, in which the authors introduce a variant of the Mean Decrease Impurity (MDI) feature importance measure aimed at overcoming the problem of MDI feature selection bias. Besides single-feature importance measures, it is worth mentioning some recent works focused on the detection of interactions between features \cite{basu2018iterative, lundberg2018consistent, devlin2019disentangled}. 

Beyond interpretability methods tailored for particular ML models, so-called \textit{model-specific} methods, there also exist several flexible approaches which earned remarkable interest due to their high portability (i.e. they can be applied to a wide range of models), so-called \textit{model-agnostic} methods. Among the most prominent model-agnostic techniques used to explain individual predictions two popular approaches are LIME \cite{ribeiro2016should} and SHAP \cite{lundberg2017unified}. Instead, Partial Dependence Plot (PDP) \cite{friedman2001greedy} and Accumulated Local Effects (ALE) plot \cite{apley2016visualizing} represent examples of model-agnostic methods used to explain the model's behavior at a global level. Exhaustive descriptions, analyses and examples of both model-specific and model-agnostic approaches can be found in \cite{guidotti2019survey, molnar2019interpretable}.

\subsection*{Interpretable Anomaly Detection}

As mentioned above, regression and classification problems (and, consequently, the models commonly used to tackle them) attract the vast majority of research interest in the XAI community. The same cannot be said for AD, unless standard ML or DL models are employed: this is typically the case where AD tasks are performed on time-series data by means of forecasting and monitoring of the missmatch between forecast and real data, that it is a formalization typically adopted for univariate AD tasks with highly non-stationary data. In the context of multivariate AD, interpretability is still a challenging topic: in the remainder of this Section we briefly describe  some of the most relevant works facing the problem of interpretability in AD. %This is not meant to be a detailed survey on the topic.

In \cite{macha2018explaining} authors aim at explaining anomalies in group. The authors introduce a new algorithm called x-PACS (which stands for eXplaining Patterns of Anomalies with Characterizing Subspaces) producing interpretable rules which are also discriminative (i.e. they can separate anomalies from the normal points) and can, thus, be used also to perform AD. 

The problems of outlier detection and outlier interpretation are addressed simultaneously also in \cite{dang2014discriminative}. The proposed algorithm is based on spectral graph embedding theory and is able to learn an optimal subspace in which an outlier is well discriminated from normal data points, while maintaining the intrinsic geometrical structure of the data for high quality outlier explanations.

In \cite{tang2015mining} a new algorithm for contextual outlier detection on categorical data is proposed. A contextual outlier is here defined as a small group of data points which share strong similarity with a larger reference group of data points on some attributes, but deviate considerably on some other attributes. In contextual outlier detection the goal is to identify the outliers, along with the associated contextual information, which is represented by: i) the corresponding reference group; ii) the attributes defining the abnormal behavior w.r.t the reference group; iii) the population of similar outliers sharing the same context and iv) the outlier degree (the ratio between the cardinality of the reference group and the cardinality of the outlier group).

Differently from the approaches described above, which rely on the design of new AD algorithms, in \cite{gupta2018beyond} the authors propose a model-agnostic method to explain outliers either detected by an AD algorithm or dictated, i.e. reported to the analyst externally. They provide compact visual explanations (respecting the limited attention of human analysts) consisting in a set of pairwise feature plots (which they call \textit{focus-plots}). Among all possible focus-plots, given a fixed budget for explanations, they select the subset of focus-plots which ``explain away" the outliers to the largest possible extent. Following a similar logic, also \cite{liu2017contextual} leverages traditional AD algorithms for the detection stage. Then, a model-agnostic Contextual Outlier INterpretation (COIN) framework is set up to provide explanations. By exploiting the isolation property of outliers, the overall problem of detector interpretation is decomposed into multiple local classification tasks aimed at explaining individual outliers. In this way, the original task turns into the problem of explaining each outlier w.r.t. its local context.

The proposed DIFFI approach, as it will be clear in the following sections, share the same ``analyst-centered" approach of \cite{gupta2018beyond} and, like in \cite{gupta2018beyond, liu2017contextual}, the focus is not on the design of a new detector. The only difference is in the scope of the proposed interpretability solutions: while the methods described in \cite{gupta2018beyond, liu2017contextual} cover a wider range of models, the DIFFI method is specifically tailored to the IF detector.



